Search for Sterile Neutrinos Mixing with Muon Neutrinos in MINOS

We report results of a search for oscillations involving a light sterile neutrino over distances of 1.04 and $735\,\mathrm{km}$ in a $\nu_{\mu}$-dominated beam with a peak energy of $3\,\mathrm{GeV}$. The data, from an exposure of $10.56\times 10^{20}\,\textrm{protons on target}$, are analyzed using a phenomenological model with one sterile neutrino. We constrain the mixing parameters $\theta_{24}$ and $\Delta m^{2}_{41}$ and set limits on parameters of the four-dimensional Pontecorvo-Maki-Nakagawa-Sakata matrix, $|U_{\mu 4}|^{2}$ and $|U_{\tau 4}|^{2}$, under the assumption that mixing between $\nu_{e}$ and $\nu_{s}$ is negligible ($|U_{e4}|^{2}=0$). No evidence for $\nu_{\mu} \to \nu_{s}$ transitions is found and we set a world-leading limit on $\theta_{24}$ for values of $\Delta m^{2}_{41} \lesssim 1\,\mathrm{eV}^{2}$.

==> mycommands.tex <==
\newcommand{\needcite}{\mbox{\color{red}{\bf {[}citation~needed}{]}}}

\newcommand{\etal}{{\it et al.}}
\newcommand{\pot}{\ensuremath{\textrm{POT}}\xspace}
\newcommand{\lepot}{\ensuremath{10.56\times10^{20}\,\pot}\xspace}
\newcommand{\lenopot}{\ensuremath{10.56\times10^{20}}\xspace}
\newcommand{\rIVpot}{\ensuremath{1.71\times10^{20}\,\pot}\xspace}
\newcommand{\rVIIpot}{\ensuremath{1.24\times10^{20}\,\pot}\xspace}
\newcommand{\baseline}{\unit[735]{km}}
\newcommand{\ndbaseline}{\unit[1.04]{km}}
\newcommand{\numi}{NuMI}
\newcommand{\annpred}{\ensuremath{49.1\pm 7.0 {\rm (stat.)} \pm 2.7 {\rm (syst.)}}}
\newcommand{\annobs}{\ensuremath{54}}
\newcommand{\limit}{\ensuremath{0.12~(0.20)}}

\newcommand{\delmsq}[1]{\ensuremath{\Delta m^2_{ #1 }}\xspace}
\newcommand{\dmsq}[1]{\ensuremath{\Delta m^2_{ #1 }}\xspace}
\renewcommand{\th}[1]{\ensuremath{\theta_{ #1 }}\xspace}
\newcommand{\sinsq}[1]{\ensuremath{\sin^{2}\!\left(2\theta_{ #1 }\right)}}
\newcommand{\sinsqdelm}[1]{\ensuremath{\sin^{2}\left(1.27\delmsq{ #1 }\frac{L}{E}\right)}}

\newcommand{\tonetwo}{\ensuremath{\theta_{12}}}
\newcommand{\tonethree}{\ensuremath{\theta_{13}}}
\newcommand{\ttwothree}{\ensuremath{\theta_{23}}}
\newcommand{\dcp}{\ensuremath{\delta_{CP}}}


\newcommand\numunue{\ensuremath{\nu_{\mu} \rightarrow \nu_{e}}}
\newcommand\numunumu{\ensuremath{\nu_{\mu} \rightarrow \nu_{\mu}}}
\newcommand\numunutau{\ensuremath{\nu_{\mu} \rightarrow \nu_{\tau}}}

\newcommand{\numu}{\ensuremath{\nu_{\mu}}\xspace}          % nu_mu
\newcommand{\numubar}{\ensuremath{\overline{\nu}_{\mu}}\xspace}   % nu_mu
\newcommand{\numucc}{\ensuremath{\nu_{\mu}}-CC\xspace} 
\newcommand{\numubarcc}{\ensuremath{\overline{\nu}_{\mu}}-CC\xspace}   % nu_mu
\newcommand {\nuecc}{\mbox{\ensuremath{\nu_{e}}-CC}\xspace}
\newcommand {\nutaucc}{\mbox{\ensuremath{\nu_{\tau}}-CC\xspace}}
\newcommand{\nus}{\ensuremath{\nu_{s}}\xspace}          % nu_s


\newcommand{\nue}{\ensuremath{\nu_{e}}\xspace}                      % nu_e
\newcommand{\nuebar}{\ensuremath{\overline{\nu}_{e}}\xspace}        % nu_e
\newcommand{\nutau}{\ensuremath{\nu_{\tau}}\xspace}              % nu_tau
\newcommand{\nutaubar}{\ensuremath{\overline{\nu}_{\tau}}\xspace}       % nu_tau
\newcommand{\anu}{\ensuremath{\overline{\nu}}}               % anu
\newcommand{\anue}{\ensuremath{\overline{\nu}_{e}}}          % anu_e
\newcommand{\anumu}{\ensuremath{\overline{\nu}_{\mu}}}       % anu_mu
\newcommand {\nux}{\ensuremath{\nu_{x}}}
\newcommand {\nubar}{\ensuremath{\bar{\nu}}}

\newcommand{\delmsqval}[2]{\ensuremath{\delmsq_{#1}=#2 {\rm eV^{2}}}}
\newcommand{\minos}{MINOS}
\newcommand{\pmns}{\ensuremath{U_{\mathrm{PMNS}}}}
\newcommand{\pmerr}[2]{\ensuremath{^{+#1}_{-#2}}}
\newcommand{\dm}{\ensuremath{\Delta m^{2}}}
\newcommand{\dmbar}{\ensuremath{ \Delta \overline{m}^{2} }\xspace}
\newcommand{\dmbarfull}{\ensuremath{\unit[\lbrack 2.62\pmerr{0.31}{0.28}\mbox{(stat.)} \pm 0.09 \mbox{(syst.)}\rbrack]{\times 10^{-3} eV^{2}}}}
\newcommand{\dmbarIV}{\ensuremath{\unit[\lbrack 3.36\pmerr{0.46}{0.40}\mbox{(stat.)} \pm 0.06 \mbox{(syst.)}\rbrack]{\times 10^{-3} eV^{2}}}}

\newcommand{\snbarIV}{\ensuremath{0.86\pm0.11 \mbox{(stat.)} \pm 0.01 \mbox{(syst.)} }}

\newcommand{\dmbarVII}{\ensuremath{\unit[\lbrack 2.26\pmerr{0.27}{0.29}\mbox{(stat.)} \pm 0.09 \mbox{(syst.)}\rbrack]{\times 10^{-3} eV^{2}}}}
\newcommand{\snbarlimitVII}{\ensuremath{0.79}\xspace}

\newcommand{\sn}{\ensuremath{\sin^{2}(2\theta)}}
\newcommand{\snbar}{\ensuremath{\sin^{2}(2\overline{\theta})}\xspace}
\newcommand{\snbarfull}{\ensuremath{0.95\pmerr{0.10}{0.11}\mbox{(stat.)} \pm 0.01 \mbox{(syst.)}}\xspace}
\newcommand{\snbarlimit}{\ensuremath{0.75}\xspace}

\newcommand{\noOscExp}{\ensuremath{273}\xspace}
\newcommand{\observedEvents}{\ensuremath{193}\xspace}
\newcommand{\exposure}{\ensuremath{2.95\times 10^{20}}\xspace}

\newcommand{\dmBestFit}{\ensuremath{2.32\times 10^{-3}eV^{2}}}
\newcommand{\snBestFit}{\ensuremath{1.0}}
\newcommand{\snLimit}{\ensuremath{0.90}\xspace}
\newcommand{\dmBestFitWithErrs}{\ensuremath{(2.32^{+0.12}_{-0.08})\times10^{-3}\,\eV^{2}}\xspace}
%\newcommand{\dmfull}{\ensuremath{\unit[ 2.32\pmerr{0.12}{0.08}\mbox{(stat.)}\pm0.09\mbox{(syst.)}]{\times 10^{-3} eV^{2}}}}
\newcommand{\dmfull}{\ensuremath{\unit[ 2.32\pmerr{0.12}{0.08}\mbox{(stat.+syst.)}]{\times 10^{-3} eV^{2}}}}

\newcommand {\comment}[1]{\textit{\color{red}{**#1**}}\xspace}
\newcommand{\unk}{\textcolor{red}{?XX?}}
\newcommand{\unc}[1]{\textcolor{magenta}{?~#1~?}}

%\newcommand{\ct}{\ensuremath{\cos\theta

